Correlation Clustering and (De)Sparsification: Graph Sketches Can Match Classical Algorithms

Correlation clustering is a widely-used approach for clustering large data sets based only on pairwise similarity information. In recent years, there has been a steady stream of better and better classical algorithms for approximating this problem. Meanwhile, another line of research has focused on porting the classical advances to various sublinear algorithm models, including semi-streaming, Massively Parallel Computation (MPC), and distributed computing. Yet, these latter works typically rely on ad-hoc approaches that do not necessarily keep up with advances in approximation ratios achieved by classical algorithms. Hence, the motivating question for our work is this: can the gains made by classical algorithms for correlation clustering be ported over to sublinear algorithms in a \emph{black-box manner}? We answer this question in the affirmative by introducing the paradigm of graph de-sparsification.

==> techniques.tex <==
\section{Techniques}

In this section, we present a brief, high-level overview of our techniques for the simplest setting of starting with a spectral sparsifier and recovering a cut sparsifier. Our approach boils down to three simple steps:
\begin{enumerate}
    \item Create a $\Ot(n)$ size linear sketch that suffices to recover a a $(1 \pm o(1))$-spectral sparsifier $H$ of $G$ (as well as recover some extra information).
    
    \item Solve a convex program to recover a {\em fractional graph} that is a $(1 \pm o(1))$- spectral sparsifier of $H$.
    
    \item Round the fractional spectral sparsifier into a simple graph that is a $(1 \pm o(1))$-cut sparsifier of $H$, and hence of $G$. 
\end{enumerate}

\paragraph{Creating the Linear Sketch:} This step is the simplest to describe. We recover three objects using $\Ot(n)$ space: a spectral sparsification linear sketch of $G$, a linear sketch for recovering low-strength edges in $G$, and the total number of edges in $G$.

\paragraph{Recovering a Fractional Spectral Sparsifier:} At this point, suppose we have opened our first sketch and recovered a $(1 \pm o(1))$ spectral sparsifier $H$ of $G$. While $H$ may have edges with polynomially large weight, we know that there exists at least one unweighted graph, namely $G$, that can serve as a spectral sparsifier of $H$. So our key observation is that we can use linear programming to find a {\em fractional unweighted} graph that is a $(1 \pm \eps)$-spectral sparsifier of $H$. Specifically, we consider the following linear program where $X$ describes a fractional graph, $m$ denotes the number of edges in $G$, and $\eps \in (0,1)$ is an arbitrarily small accuracy parameter:

 \begin{align*}
    & X_e \in [0,1] \quad \forall e \in \binom{V}{2},  \\
    & \sum_{e \in \binom{V}{2}} X_e \cdot z^T L_e z \geq (1 - \eps)z^T L_{\widetilde{G}} z \quad \forall z \in \mathbb{R}^n: \Vert z \Vert_2 = 1, \\
    & \sum_{e \in \binom{V}{2}} X_e \cdot z^T L_e z \leq (1 + \eps)z^T L_{\widetilde{G}} z \quad \forall z \in \mathbb{R}^n: \Vert z \Vert_2 = 1, \\
    & \sum_{e \in \binom{V}{2}} X_e = m.
\end{align*}

Importantly, because the original graph $G$ is in this linear space (as are small perturbations of $G$), the solution space of this linear program is non-empty. Moreover, given any fractional solution $X \in [0,1]^{\binom{V}{2}}$, we can verify in polynomial-time it to be either feasible or find a violated constraint as this task essentially reduces to checking the spectrum of a graph Laplacian. We thus have a polynomial-time separation oracle for this program, and can find a feasible solution, say $\widetilde{H}$, in polynomial-time using the ellipsoid method.

\paragraph{Randomized Rounding:} Finally, we need to recover an unweighted simple graph $G'$ from $\widetilde{H}$ that is a a $(1 \pm \eps)$-cut sparsifier of $G$. A natural approach would be to simply include each edge $e$ in $G'$ with probability $X_e$, preserving the size of each cut in {\em expectation}. But the challenge is to ensure that this expected behavior holds for every cut. 

This is similar to the issue handled by Karger in his work on cut sparsifiers~\cite{Kar93}, and one can show that the randomized rounding works provided 
the minimum cut in the graph $G$ is at least $C \log(n) / \eps^2$ for some sufficiently large constant $C$. Our final ingredient now comes into play: we store a linear sketch of size $\Ot(n)$ which recovers exactly the set of edges $F$ in $G$ with ``strength'' $< C \log(n) / \eps^2$. Once we remove these low strength edges, the graph is disconnected into components each of which has a minimum cut of size $\geq C \log(n) / \eps^2$. We now instead recover the spectral sparsifier of the graph $G - F$ using linearity of our sketch, and run the convex program in the second step as before. Now in the rounding step, we are guaranteed that all the cut sizes concentrate, thus yielding a $(1 \pm \eps)$ cut-sparsifier of our graph $G$ once we add back the edges in $F$.

There is one final issue that remains: in order to preserve the values of the correlation clustering objective, it does not suffice to simply be a cut-sparsifier. Rather, a graph must \emph{both} be a cut-sparsifier and have the same number of edges as the original graph. To achieve this additional property, we observe that each edge contributes an independent $\mathrm{Bern}(X_e)$ to the total number of edges. Thus, the distribution of the total edge mass in the rounded graph is $\sum_{e \in \widetilde{H}} \mathrm{Bern}(X_e)$, and by the constraint of our convex program, the expected size is exactly $m$. In a single round of rounding, we have no guarantee that we get exactly $m$ edges surviving. However, exploiting the fact that the rounding outputs a cut sparsifier with high probability, we can \emph{repeatedly round} some $\mathrm{poly}(n)$ number of times and guarantee that \emph{in at least one of these rounds}, the number of surviving edges is exactly $m$. This allows us to finally recover a graph $G'$ that is both a $(1 \pm \eps)$-cut sparsifier of $G$ and has exactly the same number of edges as $G$.

